Simplification of cross-field topology

We present an innovative algorithm that simplifies the topology of a cross-field. Our algorithm works through macro-operations that allow us editing the graph of separatrices, which is extracted from a cross-field, while maintaining it topologically consistent. We present preliminary results of our implementation.

==> disilogo.tex <==
\font\disifont=cmsy10 scaled \magstep 3
\newbox\Ball
\setbox\Ball=\hbox{\disifont\char"0F}
\newdimen\BB \BB=\wd\Ball
\advance\BB by -.22\BB
\newbox\dSB
\setbox\dSB=\hbox{\vrule height.5\BB width.5\BB}
\newbox\dVB
\setbox\dVB=\hbox{\vrule height\BB width.2\BB}
\newbox\dHB
\setbox\dHB=\hbox{\vrule height.2\BB width\BB}
\newbox\dWB
\setbox\dWB=\hbox to .02\BB{\hss\vrule height1.01\BB width.04\BB\hss}

\setbox\Ball=\hbox to 0pt{\hss\vbox to 0pt{\vss\kern.135\BB\hbox{\disifont\char"0F}\vss}\hss}

\def\TL{\hbox to 0pt{\hss\vbox to 0pt{\vss\copy\dSB}}}
\def\TR{\hbox to 0pt{\vbox to 0pt{\vss\copy\dSB}\hss}}
\def\BL{\hbox to 0pt{\hss\vbox to 0pt{\copy\dSB\vss}}}
\def\BR{\hbox to 0pt{\vbox to 0pt{\copy\dSB\vss}\hss}}
\def\SquareBrick#1#2#3#4{\vbox to \BB{\vss\hbox to \BB{\hss #1#2#3#4\hss}\vss}}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\vbox{#1}\vrule}\hrule}}
\def\WB#1{\raise#1\BB\copy\dWB}

\def\DISIwave{\boxit{\hbox to 3.4\BB
      {\SquareBrick\TL\TR\BL\BR
       \WB{.005}\WB{.01}\WB{.02}\WB{.04}\WB{.07}\WB{.11}\WB{.14}\WB{.20}%
       \WB{.27}\WB{.35}\WB{.45}\WB{.55}\WB{.65}\WB{.75}\WB{.83}\WB{.90}\WB{.96}%
       \WB{1.01}\WB{1.06}\WB{1.10}\WB{1.13}\WB{1.15}\WB{1.16}\WB{1.17}\WB{1.18}%
       \WB{1.18}\WB{1.17}\WB{1.14}\WB{1.10}\WB{1.03}\WB{.91}\WB{.75}\WB{.50}%
       \WB{.25}\WB{0}\WB{-.25}\WB{-.50}\WB{-.75}\WB{-.91}\WB{-1.03}\WB{-1.10}%
       \WB{-1.14}\WB{-1.17}\WB{-1.18}\WB{-1.19}\WB{-1.20}\WB{-1.19}\WB{-1.18}%
       \WB{-1.16}\WB{-1.15}\WB{-1.13}\WB{-1.10}\WB{-1.06}\WB{-1.01}\WB{-.96}%
       \WB{-.90}\WB{-.83}\WB{-.75}\WB{-.65}\WB{-.55}\WB{-.45}\WB{-.35}\WB{-.27}%
       \WB{-.18}\WB{-.12}\WB{-.08}\WB{-.05}\WB{-.04}\WB{-.03}\WB{-.025}%
       \SquareBrick\TL\TR\BL\BR\hss}}}

\def\DISIlogo{\hbox to 13.8\BB{\baselineskip=0pt 
\DISIwave\hfill
\hbox{% letter D
 \vbox to 3.4\BB{%
 \hbox{\SquareBrick\TL\TR\BL\BR
        \copy\dVB
         \SquareBrick\TL\TR\BL\BR
          \copy\dVB
           \SquareBrick\TL\BR\BL{\copy\Ball}}\vss
 \hbox{\copy\dHB
        \kern1.4\BB
         \copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BL\BR
        \kern1.4\BB
         \SquareBrick\TL\TR\BL\BR}\vss
 \hbox{\copy\dHB
        \kern1.4\BB
         \copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BL\BR
        \copy\dVB
         \SquareBrick\TL\TR\BL\BR
          \copy\dVB
           \SquareBrick\TL\TR\BL{\copy\Ball}}%
}}\kern .2\BB
\hbox{% letter I
 \vbox to 3.4\BB{%
 \hbox{\SquareBrick\TL\TR\BL\BR}\vss
 \hbox{\copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BL\BR}\vss
 \hbox{\copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BR{\copy\Ball}}%
}}%
\hbox{% link I_S
 \vbox to 3.4\BB{\vss
 \hbox{\copy\dVB}%
}}%
\hbox{% letter S
 \vbox to 3.4\BB{%
 \hbox{\SquareBrick\TR\BL\BR{\copy\Ball}%
        \copy\dVB
         \SquareBrick\TL\TR\BL\BR
          \copy\dVB
           \SquareBrick\TL\BR\BL\TR}\vss
 \hbox{\copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BR{\copy\Ball}%
        \copy\dVB
         \SquareBrick\TL\TR\BL\BR
          \copy\dVB
           \SquareBrick\TL\BL\BR{\copy\Ball}}\vss
 \hbox{\kern 2.4\BB
        \copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BR\BL
        \copy\dVB
         \SquareBrick\TL\TR\BL\BR
          \copy\dVB
           \SquareBrick\TL\TR\BL{\copy\Ball}}%
}}\kern .2\BB
\hbox{% letter I
 \vbox to 3.4\BB{%
 \hbox{\SquareBrick\TL\TR\BL\BR}\vss
 \hbox{\copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BL\BR}\vss
 \hbox{\copy\dHB}\vss
 \hbox{\SquareBrick\TL\TR\BR\BL}%
}}%
}}

